Egocentric Video-Language Pretraining @ EPIC-KITCHENS-100 Multi-Instance Retrieval Challenge 2022

In this report, we propose a video-language pretraining (VLP) based solution \cite{kevin2022egovlp} for the EPIC-KITCHENS-100 Multi-Instance Retrieval (MIR) challenge. Especially, we exploit the recently released Ego4D dataset \cite{grauman2021ego4d} to pioneer Egocentric VLP from pretraining dataset, pretraining objective, and development set. Based on the above three designs, we develop a pretrained video-language model that is able to transfer its egocentric video-text representation to MIR benchmark. Furthermore, we devise an adaptive multi-instance max-margin loss to effectively fine-tune the model and equip the dual-softmax technique for reliable inference. Our best single model obtains strong performance on the challenge test set with 47.39% mAP and 61.44% nDCG. The code is available at https://github.com/showlab/EgoVLP.

==> tex/epic_vis.tex <==
\begin{figure*}[htb]
\centering
\vspace{-0.3cm}
\centering
\includegraphics[width=1.0\linewidth]{figures/epic_vis.pdf}
\label{case_1}
\centering
\vspace{-0.3cm}
\caption{Visualization of \epic~text-video retrieval. 
Given the same text query, we compare the \textbf{Top-5 results} of 1st-person pretraining and 3rd-person pretraining.}
\label{fig_epic_vis}
\end{figure*}
